Vocal Tract Length Warped Features for Spoken Keyword Spotting

In this paper, we propose several methods that incorporate vocal tract length (VTL) warped features for spoken keyword spotting (KWS). The first method, VTL-independent KWS, involves training a single deep neural network (DNN) that utilizes VTL features with various warping factors. During training, a specific VTL feature is randomly selected per epoch, allowing the exploration of VTL variations. During testing, the VTL features with different warping factors of a test utterance are scored against the DNN and combined with equal weight. In the second method scores the conventional features of a test utterance (without VTL warping) against the DNN. The third method, VTL-concatenation KWS, concatenates VTL warped features to form high-dimensional features for KWS. Evaluations carried out on the English Google Command dataset demonstrate that the proposed methods improve the accuracy of KWS.

==> references <==
@article{lopez2021deep,
  title={Deep spoken keyword spotting: An overview},
  author={L{\'o}pez-Espejo, I. and Tan, Z.-H. and Hansen, JHL and Jensen, J.},
  journal={IEEE Access},
  volume={10},
  pages={4169--4199},
  year={2021},
  publisher={IEEE}
}

@INPROCEEDINGS{1325931,
  author={Xu Shao and Milner, B.},
  booktitle={2004 IEEE International Conference on Acoustics, Speech, and Signal Processing}, 
  title={Pitch prediction from MFCC vectors for speech reconstruction}, 
  year={2004},
  volume={1},
  number={},
  pages={I-97},
  doi={10.1109/ICASSP.2004.1325931}}
  
  @ARTICLE{6923432, 
  author={Han, Kun and Wang, DeLiang},  
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  title={Neural Network Based Pitch Tracking in Very Noisy Speech},
  year={2014},
  volume={22},
  number={12}, 
  pages={2158-2168}, 
  doi={10.1109/TASLP.2014.2363410}
  }
  
  @inproceedings{Tran2020,
  author={D. N. Tran and U. Batricevic and K. Koishida},
  title={{Robust Pitch Regression with Voiced/Unvoiced Classification in Nonstationary Noise Environments}},
  year=2020,
  booktitle={Proc. Interspeech 2020},
  pages={175--179},
  doi={10.21437/Interspeech.2020-3019},
  url={http://dx.doi.org/10.21437/Interspeech.2020-3019}
}


@ARTICLE{PEFAC,
author ={S. Gonzalez and M. Brookes}, 
title = {PEFAC - a pitch estimation algorithm robust to high levels of noise},
journal = {IEEE Trans. Audio, Speech, Language Processing},
volume = {22},
number = {2},
pages = {518-530},
year = {2014}
}
       

@inproceedings{Chung2019,
  author={Y. Chung and W.-N. Hsu and H. Tang and J. Glass},
  title={{A}n Unsupervised Autoregressive Model for Speech Representation Learning},
  year=2019,
  booktitle={Proc. Interspeech},
  pages={146--150},
  }
  
  @inproceedings{chung2020generative,
  title = {{G}enerative pre-training for speech with auto-regressive predictive coding},
  author = {Chung, Y.-A. and Glass, J.},
  booktitle = {Proc of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  year = {2020},
  pages={3497-3501}
}

@article{TanSD20,
  author    = {Z.-H. Tan and  A. K. Sarkar and N. Dehak},
  title     = {{rVAD}: An Unsupervised Segment-based Robust Voice Activity Detection Method},
  journal   = {Computer Speech \& Language},
  volume    = {59},
  pages     = {1--21},
  year      = {2020}
 } 
 
 @inproceedings{LPC,
 author = {B. S. Atal and J. Remde},
 title={{A} new model of LPC excitation for producing natural-sounding speech at low bit rates}, 
 booktitle = {Proc of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 year ={1982},
 pages = {614–617}
 }
 
 
 @Article{Sohn1999a,
author={J. Sohn and N. S. Kim and W. Sung},
title={{A} statistical model-based voice activity detection},
journal={IEEE Signal Processing Letters},
volume={6},
number = {1},
pages={1-3},
year={1999}
}

@inproceedings{VQVAD,
author={T. Kinnunen and P. Rajan},
title={{A} practical, self-adaptive voice activity detector for speaker verification with noisy telephone and microphone
data},
booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2013}
}


@article{DBLP:journals/csl/SarkarT21,
  author    = {A. K. Sarkar and  Z.-H. Tan},
  title     = {{S}elf-segmentation of pass-phrase utterances for deep feature learning in text-dependent speaker verification},
  journal   = {Computer Speech \& Lang.},
  volume    = {70},
  pages     = {101229},
  year      = {2021}
  }
  
  
  @ARTICLE{FITPUB11518,
   author = "R. F\'{e}r and P. Mat\v{e}jka and F. Gr\'{e}zl and O. Plchot and K. Vesel\'{y} and J. \v{C}ernock\'{y}",
   title = "{M}ultilingually Trained Bottleneck Features in Spoken Language Recognition",
   pages = "252--267",
   journal = "Computer Speech and Language",
   volume = 2017,
   number = 46,
   year = 2017
   }
   
   
  @article{DBLP:journals/corr/abs-2107-10790,
  author    = {J. M. M. Torres and
               M. Ravanelli and
               S. E. Medina{-}DeVilliers and
               M. D. Lerner and
               G. Riccardi},
  title     = {{I}nterpretable SincNet-based Deep Learning for Emotion Recognition from {EEG} brain activity},
    year      = {2021},
  url       = {https://arxiv.org/abs/2107.10790},
  eprinttype = {arXiv}
  
  }


@Article{bonastre04,
  author="J. F. Bonastre and et. al",
  title="NIST'04 Speaker Rcognition Evaluation Campaign: New LIA Speaker Detection {P}lateform based on {ALIZE} {T}oolkit",
  journal="in NIST SRE'04 Workshop, Toledo, Spain",
   year="2004"
  }

@INPROCEEDINGS{Povey_ASRU2011,
         author = {Povey, Daniel and others},
           title = {The Kaldi Speech Recognition Toolkit},
      booktitle = {Proc. of IEEE Workshop on Automatic Speech Recognition and Understanding},
           year = {2011}
}

@misc{yu2020waveformbased,
      title={Waveform-based Voice Activity Detection Exploiting Fully Convolutional networks with Multi-Branched Encoders}, 
      author={C. Yu and K.-H. Hung and I-F. Lin and S.-W. Fu and Y. Tsao and J.-W. Hung},
      year={2020},
      eprint={2006.11139},
      archivePrefix={arXiv}
      
}


@inproceedings{vafeiadis19_interspeech,
  author={A. Vafeiadis and E. Fanioudakis and I. Potamitis and K. Votis and D. Giakoumis and D. Tzovaras and L. Chen and R. Hamzaoui},
  title={{T}wo-Dimensional Convolutional Recurrent Neural Networks for Speech Activity Detection},
  year=2019,
  booktitle={Proc.of Interspeech},
  pages={2045--2049}
  
}

@Article{Yuan2015,
author={Y. Liu and Y. Qian and N. Chen and T. Fu and Y. Zhang and K. Yu},
title= {{D}eep {F}eature {F}or {T}ext-dependent {S}peaker {V}erification},
journal={Speech Communication},
volume={73},
pages={1-13},
year={2015}
}

@article{DBLP:journals/taslp/SarkarTTSG19,
  author    = {A. K. Sarkar and Z. -H. Tan and H. Tang and S. Shon and  J. R. Glass},
  title     = {Time-Contrastive {L}earning {B}ased {D}eep {B}ottleneck {F}eatures for {T}ext-Dependent {S}peaker {V}erification},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {27},
  number    = {8},
  pages     = {1267--1279},
  year      = {2019}
}

@inproceedings{McLaren2015,
author={M. McLaren and Y. Lei and L. Ferrer},
title={{A}dvances {I}n {D}eep {N}eural {N}etwork {A}pproaches {T}o {S}peaker {R}ecognition},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2015}
}

@inproceedings{Hinton2012,
author = {G. Hinton and others},
title = {{D}eep {N}eural {N}etworks {F}or {A}coustic {M}odeling {I}n {S}peech {R}ecognition},
booktitle={IEEE Signal Process. Mag.},
pages={82-97},
year={2012}
}

@Article{RSR2015,
author={A. Larcher and  K. A. Lee and  B. Ma and H. Li},
title= {{T}ext-dependent speaker verification: classifiers, databases and RSR2015},
journal={Speech Communucation},
volume={60},
pages={56-77},
year={2014}
}


@inproceedings{Hirsch2000,
author ={ H.-G. Hirsch and D. Pearce},
title = {{T}HE AURORA EXPERIMENTAL FRAMEWORK FOR THE PERFORMANCE EVALUATION OF SPEECH RECOGNITION SYSTEMS UNDER NOISY CONDITIONS},
booktitle ={Automatic Speech Recognition: Challenges for the Next Millennium, ISCA ITRW ASR2000},
year= {2000}
}

@misc{musan2015,
  author = {D. Snyder and G. Chen and D. Povey},
  title = {{MUSAN}: A Music, Speech, and Noise Corpus},
  year = {2015},
  eprint = {1510.08484},
  note = {arXiv:1510.08484v1}
}


@inproceedings{DBLP:journals/corr/HendrycksG16-old,
  author    = {D. Hendrycks and   K. Gimpel},
  title     = {{B}ridging Nonlinearities and Stochastic Regularizers with Gaussian  Error Linear Units},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.08415},
  archivePrefix = {arXiv}
 }
 
 
 @inproceedings{hansen19_interspeech,
  author={J. H.L. Hansen and A. Joglekar and M. C. Shekhar and V. Kothapally and C. Yu and L. Kaushik and A. Sangwan},
  title={{The 2019 Inaugural Fearless Steps Challenge: A Giant Leap for Naturalistic Audio}},
  year=2019,
  booktitle={Proc. Interspeech},
  pages={1851-1855}
 }
 
 @INPROCEEDINGS{kraljevski2015comparison,
  title={Comparison of forced-alignment speech recognition and humans for generating reference VAD},
  author={Kraljevski, Ivan and Tan, Zheng-Hua and Bissiri, Maria Paola},
  booktitle ={Proc. of Interspeech},
  year={2015},
  pages= {2937-941}
  }
  
  
  @inproceedings{Hansen2019,
  author={J. H.L. Hansen and A. Joglekar and M. C. Shekhar and V. Kothapally and C. Yu and L. Kaushik and A. Sangwan},
  title={{T}he 2019 Inaugural Fearless Steps Challenge: A Giant Leap for Naturalistic Audio},
  year=2019,
  booktitle={Proc. of Interspeech},
  pages={1851--1855}
  }
  
  
  
@inproceedings{ko15_interspeech,
  author={T. Ko and V. Peddinti and D. Povey and S. Khudanpur},
  title={{A}udio augmentation for speech recognition},
  year=2015,
  booktitle={Proc. Interspeech},
  pages={3586-3589}
  
}

@inproceedings{Wang2020,
author = {G. Wang and  A. Rosenberg and Z. Chen and Y. Zhang and B. Ramabhadran},
title = {{I}mproving speech recognition using consistent predictions on synthesized speech},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year = {2020},
pages = {7029-7033}
}

@inproceedings{park19e_interspeech,
  author={D. S. Park and W. Chan and Y. Zhang and C.-C. Chiu and B. Zoph and E. D. Cubuk and Q. V. Le},
  title={{S}pecAugment: A Simple Data Augmentation Method for Automatic Speech Recognition},
  year=2019,
  booktitle={Proc. Interspeech},
  pages={2613-2617}
  }
  
  @article{Hermansky1990,
    author = {Hermansky, H.},
    journal = {Journal of the Acoustical Society of America},
     number = 4,
    pages = {1738-1752},
    title = {{P}erceptual linear predictive (PLP) analysis of speech},
    volume = 87,
    year = 1990
   }

@Article{Davis80,
	author={S. B. Davis and P. Mermelstein},
	title={{C}omparison of parametric representations for monosyllabic word recognition in continuously spoken sentences},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={28},
	pages={357-366},
	year={1980}
}

@inproceedings{Larsen22,
author= {C.M. Larsen and P. Koch and Z.-H. Tan.},
title={{A}dversarial Multi-Task Deep Learning for Noise-Robust Voice Activity Detection with Low Algorithmic Delay},
year ={2022},
booktitle={Submitted to Interspeech}
}

@inproceedings{Ryant2013SpeechAD,
  title={Speech activity detection on youtube using deep neural networks},
  author={N. Ryant and M. Y. Liberman and J. Yuan},
  booktitle={INTERSPEECH},
  year={2013}
}


@INPROCEEDINGS{6639096,  
author={Hughes, T. and Mierle, K.},  
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},  
title={{R}ecurrent neural networks for voice activity detection}, 
year={2013},  
pages={7378-7382}
}

@INPROCEEDINGS{6637694,  
author={Eyben, F. and Weninger, F. and Squartini, S. and Schuller, B.},  booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)}, 
title={{R}eal-life voice activity detection with LSTM Recurrent Neural Networks and an application to Hollywood movies},  
year={2013},  
pages={483-487}
}

@INPROCEEDINGS{7868454,  
author={J. Pang},  
booktitle={EEE Annual Computing and Communication Workshop and Conference (CCWC)},   
title={{S}pectrum energy based voice activity detection},   
year={2017},  
pages={1-5}
}

@INPROCEEDINGS{Wave_2020,
  author = {Yu, C. and Hung, K.-H. and Lin, I-F. and Fu, S.-W. and Tsao, Y. and Hung, J.-W.},
  title = {{W}aveform-based Voice Activity Detection Exploiting Fully Convolutional networks with Multi-Branched Encoders},
   booktitle= {arXiv},
  year = {2020}
  }
  
  
@techreport{ITU1996,
  author      = "A. Itu",
  title       = "{S}ilence compression scheme for g. 729 optimized for terminals conforming to recommendation v. 70",
  institution = "ITU-T Recommendation G vol. 729",
  year        = "1996"
}
  
@Article{Sohn1999,
author = "J. Sohn and N. S. Kim and W. Sung",
title= {{A} statistical model-based voice activity detection},
journal = {IEEE signal processing letters},
volume= {6},
number = {1},
pages = {1-3},
year = { 1999}
}

@ARTICLE{1510660,
  author={Ramirez, J. and Segura, J.C. and Benitez, C. and Garcia, L. and Rubio, A.},
  journal={IEEE Signal Processing Letters}, 
  title={{S}tatistical voice activity detection using a multiple observation likelihood ratio test}, 
  year={2005},
  volume={12},
  number={10},
  pages={689-692},
}

@ARTICLE{5546913,
  author={Yu, Tao and Hansen, John H. L.},
  journal={IEEE Signal Processing Letters}, 
  title={{D}iscriminative Training for Multiple Observation Likelihood Ratio Based Voice Activity Detection}, 
  year={2010},
  volume={17},
  number={11},
  pages={897-900}
  }

@article{HWANG20161,
author = {I. Hwang and H.-M. Park and J.-H. Chang },
title = {{E}nsemble of deep neural networks using acoustic environment classification for statistical model-based voice activity detection},
journal = {Computer Speech \& Language},
volume = {38},
pages = {1-12},
year = {2016}
}

@ARTICLE{5873124,
  author={Wu, J. and Zhang, X.-L.},
  journal={IEEE Signal Processing Letters}, 
  title={{E}fficient Multiple Kernel Support Vector Machine Based Voice Activity Detection}, 
  year={2011},
  volume={18},
  number={8},
  pages={466-469}
  }

@ARTICLE{7347379,  
author={Zhang, X.-L. and Wang, D.}, 
journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
title={Boosting Contextual Information for Deep Neural Network Based Voice Activity Detection},  
year={2016},  volume={24},  number={2},  pages={252-264}
}

@ARTICLE{6905738,
  author={Chen, J. and Wang, Y. and Wang, D.},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={{A} Feature Study for Classification-Based Speech Separation at Low Signal-to-Noise Ratios}, 
  year={2014},
  volume={22},
  number={12},
  pages={1993-2002}
}
  
@inproceedings{Dean2015TheQP,
  title={The QUT-NOISE-SRE protocol for the evaluation of noisy speaker recognition},
  author={David Dean and Ahilan Kanagasundaram and Houman Ghaemmaghami and Md. Hafizur Rahman and Sridha Sridharan},
  booktitle={Interspeech},
  year={2015}
}


@ARTICLE{8309294,
  author={Kim, J. and Hahn, M.},
  journal={IEEE Signal Processing Letters}, 
  title={Voice Activity Detection Using an Adaptive Context Attention Model}, 
  year={2018},
  volume={25},
  number={8},
  pages={1181-1185}
  }

@misc{xue2022ecapatdnn,
      title={ECAPA-TDNN for Multi-speaker Text-to-speech Synthesis}, 
      author={J. Xue and Y. Deng and Y. Han and Y. Li and J. Sun and J. Liang},
      year={2022},
      archivePrefix={arXiv}
      
}


@inproceedings{Dawalatabad2021ECAPATDNNEF,
  title={ECAPA-TDNN Embeddings for Speaker Diarization},
  author={N. Dawalatabad and M. Ravanelli and F. Grondin and J. Thienpondt and B. Desplanques and H. Na},
  booktitle={Proc of Interspeech},
  year={2021}
  }

@inproceedings{myer2018efficient,
      title={Efficient keyword spotting using time delay neural networks}, 
      author={S. Myer and V. S. Tomar},
      year={2018},
      booktitle={Proc of Interspeech},
      pages = {1264-1268}
}

@inproceedings{lv2023dccrnkws,
      title={DCCRN-KWS: an audio bias based model for noise robust small-footprint keyword spotting}, 
      author={S. Lv and X. Wang and S. Sun and L. Ma and L. Xie},
      year={2023},
      booktitle={Proc of Interspeech},
      pages = {929-933}
}


@inproceedings{Parnami_2022,
   title={Few-Shot Keyword Spotting With Prototypical Networks},
   DOI={10.1145/3529399.3529443},
   booktitle={International Conference on Machine Learning Technologies (ICMLT)},
   author={Parnami, A. and Lee, M.},
   year={2022}
}


@inproceedings{Rybakov_2020, 
   title={Streaming Keyword Spotting on Mobile Devices},
   DOI={10.21437/interspeech.2020-1003},
   booktitle={Proc of Interspeech},
   author={Rybakov, O. and Kononenko, N. and Subrahmanya, N. and Visontai, M. and Laurenzo, S.},
   year={2020},
   pages = {2277-2281}
}

@INPROCEEDINGS{Jaitly_vocaltract,
    author = {N. Jaitly and G. E. Hinton},
    title = {{V}ocal Tract Length Perturbation VTLP Improves Speech Recognition},
    booktitle = {Proc. of International Conference on Machine Learning (ICML)},
    year = {2013}
}

@article{speechcommandsv2-temp,
   author = { {Warden}, P.},
    title = "{Speech Commands: A Dataset for Limited-Vocabulary Speech Recognition}",
  journal = {ArXiv e-prints},
   eprint = {1804.03209},
year = 2018   
}

@article{speechcommandsv2,
  title={Speech commands: A dataset for limited-vocabulary speech recognition},
  author={Warden, Pete},
  journal={arXiv preprint arXiv:1804.03209},
  year={2018}
}



@Article{htkbook,
  author="S. Young and D. Kershaw and J. Odell and V. Valtchev and P. Woodland and et al.",
  title="{HTK} book",
  journal={Copyright 2001-2006 Cambridge University Engineering Department}
   }

@INPROCEEDINGS{deandrade2018neural,
      title={A neural attention model for speech command recognition}, 
      author={D. C. D. Andrade and S. Leo and M. L. D. S. Viana and C. Bernkopf},
      year={2018},
       booktitle={arXiv}   
}

@misc{he2015deep,
      title={Deep Residual Learning for Image Recognition},
      author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
      year={2015},
      eprint={1512.03385},
      booktitle={arXiv}      
}

@INPROCEEDINGS{librosa,
author = {M. Brian and C. Raffel and D. Liang and D. P. Ellis and M. McVicar and E. Battenberg and Oriol Nieto},
title={librosa: Audio and music signal analysis in python},
booktitle={Proc. of the 14th python in science conference},
pages = {18-25},
year = {2015}
}

@inproceedings{choi2019temporal,
      title={Temporal Convolution for Real-time Keyword Spotting on Mobile Devices}, 
      author={S. Choi and others},
      year={2019},
    booktitle={Proc. of Interspeech},
  pages={3372--3376}
     
      
}

@inproceedings{Berg_2021, 
   title={Keyword Transformer: A Self-Attention Model for Keyword Spotting},
   booktitle={Proc of Interspeech},
   author={Berg, A. and O’Connor, M. and Cruz, M. T.},
   year={2021},
   pages={4249--4253}
}

@INPROCEEDINGS{7078563,
  author={Serizel, R. and Giuliani, D.},
  booktitle={Proc. of IEEE Spoken Language Technology Workshop (SLT)}, 
  title={Vocal tract length normalisation approaches to DNN-based children's and adults' speech recognition}, 
  year={2014},
    pages={135-140}
 }

@inproceedings{akhil-interspeech2008,
      author = {P. T. Akhil and S. P. Rath and S. Umesh and D. R. Sanand},
      title = {{A} computationally efficient approach to warp factor estimation in VTLN using EM algorithm and sufficient satistics},
      booktitle = {Proc. of Interspeech},
      pages = {1713-1716},
      year = {2008}
}

@article{Lee-Rose98,
      author="L. Lee and R. Rose",
      title="{F}requency warping approach  to speaker normalization",
      journal="IEEE Trans. on Speech and Audio Processing",
      volume={6},
      pages={49-59},
      year={1998}
}

@INPROCEEDINGS{7178863,
  author={Prabhavalkar, R. and others},
  booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)}, 
  title={Automatic gain control and multi-style training for robust small-footprint keyword spotting with deep neural networks}, 
   year={2015},
    pages={4704-4708}
  }
@InProceedings{FRSM12_TelephonicSpeech,
author="Basu, J.
and Bepari, M. S.
and Roy, R.
and Khan, S.",
title="Design of Telephonic Speech Data Collection and Transcription Methodology for Speech Recognition Systems",
booktitle="Proc. of FRSM",
year="2012",
address="India",
pages="147--153"
}


@inproceedings{kim21l_interspeech,
  author={B. Kim and S. Chang and J. Lee and D. Sung},
  title={Broadcasted Residual Learning for Efficient Keyword Spotting},
  year=2021,
  booktitle={Proc. of Interspeech},
  pages={4538--4542}
  
}

@inproceedings{paszke2017automatic,
  title={Automatic differentiation in PyTorch},
  author={Paszke, A. and others},
  booktitle={Proc. of Neural Information Processing Systems (NIPS)},
  year={2017}
}



@inproceedings{mørk2024noiserobustkeywordspottingselfsupervised-temp,
      title={Noise-Robust Keyword Spotting through Self-supervised Pretraining}, 
      author={J. Mørk and H. S. Bovbjerg and G. Kiss and Z.-H. Tan},
      year={2024},
      booktitle={arXiv}      
}

@article{mrk2024noiserobustkeywordspottingselfsupervised,
  title={Noise-Robust Keyword Spotting through Self-supervised Pretraining},
  author={M{\o}rk, Jacob and Bovbjerg, Holger Severin and Kiss, Gergely and Tan, Zheng-Hua},
  journal={arXiv preprint arXiv:2403.18560},
  year={2024}
}

@ARTICLE{10607847,
  author={Shi, Y. and Li, L. and Wang, D. and Han, J.},
  journal={IEEE Signal Processing Letters}, 
  title={Keyword Guided Target Speech Recognition}, 
  year={2024},
  volume={31},
  pages={1945-1949}
  }

@inproceedings{yusuf2024pretrainingendtoendkeywordsearch-temp,
      title={Pretraining End-to-End Keyword Search with Automatically Discovered Acoustic Units}, 
      author={B. Yusuf and J. H. Černocký and M. Saraçlar},
      year={2024},
      booktitle={arXiv}      
}

@article{yusuf2024pretrainingendtoendkeywordsearch,
  title={Pretraining End-to-End Keyword Search with Automatically Discovered Acoustic Units},
  author={Yusuf, Bolaji and {\v{C}}ernock{\`y}, Jan and Sara{\c{c}}lar, Murat and others},
  journal={arXiv preprint arXiv:2407.04652},
  year={2024}
}

@inproceedings{sarkar09_interspeech,
  title     = {Text-independent speaker identification using vocal tract length normalization for building universal background model},
  author    = {A. K. Sarkar and S. Umesh and S. P. Rath},
  year      = {2009},
  booktitle = {Proc. of Interspeech},
  pages     = {2331-2334}
  }

@ARTICLE{9339931,
  author={Sarkar, A. K. and Tan, Z.-H.},
  journal={IEEE Signal Processing Letters}, 
  title={Vocal Tract Length Perturbation for Text-Dependent Speaker Verification With Autoregressive Prediction Coding}, 
  year={2021},
  volume={28},
  number={},
  pages={364-368}
  }
@article{MADHAVI2019175,
title = {Vocal Tract Length Normalization using a Gaussian mixture model framework for query-by-example spoken term detection},
journal = {Computer Speech \& Language},
volume = {58},
pages = {175-202},
year = {2019},
author = {M. C. Madhavi and H. A. Patil}}

@INPROCEEDINGS{5700849,
  author={Szöke, I and Grézl, F. and Černocký, J. and Fapšo, M. and Cipr, T.},
  booktitle={Proc. of IEEE Spoken Language Technology Workshop}, 
  title={Acoustic keyword spotter - optimization from end-user perspective}, 
  year={2010},
  pages={189-193}
}

